SEval-NAS: A Search-Agnostic Evaluation for Neural Architecture Search

Neural architecture search (NAS) automates the discovery of neural networks that meet specified criteria, yet its evaluation procedures are often hardcoded, limiting the ability to introduce new metrics. This issue is especially pronounced in hardware-aware NAS, where objectives depend on target devices such as edge hardware. To address this limitation, we propose SEval-NAS, a metric-evaluation mechanism that converts architectures to strings, embeds them as vectors, and predicts performance metrics. Using NATS-Bench and HW-NAS-Bench, we evaluated accuracy, latency, and memory. Kendall's $\tau$ correlations showed stronger latency and memory predictions than accuracy, indicating the suitability of SEval-NAS as a hardware cost predictor. We further integrated SEval-NAS into FreeREA to evaluate metrics not originally included. The method successfully ranked FreeREA-generated architectures, maintained search time, and required minimal algorithmic changes. Our implementation is available at: https://github.com/Analytics-Everywhere-Lab/neural-architecture-search

==> content/5_results.tex <==
\section{Results and Discussion}
% [MERGE RESULTS INTO EXPERIMENTS AND RESULTS]

This section provides a correlation analysis of predicted vs. actual metrics for test sets for each benchmark dataset. Each comparison is assessed using Kendall Tau and Pearson's correlation coefficients. Kendall Tau correlation coefficient is frequently used in evaluating NAS frameworks and benchmarks \cite{LiC2021} \cite{Mellor2021}. Correlation values closer to +1 indicate stronger positive associations, while values closer to 0 indicate weaker associations. 

\subsection{NATS-Bench}
We trained the evaluator on the topology search space (TSS) and size search spaces (SSS) of the NATS-Bench benchmark for separate \texttt{(accuracy, memory)} and \texttt{(accuracy, latency)} objective pairs. 

Figure \ref{} presents the results for both objectives in the TSS search space. For the \texttt{(accuracy, memory)} objective pair, there was a moderate positive correlation ($\tau = 0.5266$) between the predicted and true test accuracies and a strong positive correlation ($\tau = 0.8753$) between predicted and true memory values. The \texttt{(accuracy, latency)} objective pair paints a similar picture, where accuracy has a moderate positive correlation ($\tau = 0.5308$) and latency has a strong positive correlation ($\tau = 0.8068$).

% INCLUDE PARETO RESULTS FOR BOTH AND DISCUSS IT

The results for the size search space (SSS) are shown in Figure \ref{}. Similar to the TSS results, the accuracy correlation is moderate ($\tau = 0.5760$), and memory usage has a strong positive correlation ($\tau = 0.9570$) for the \texttt{(accuracy, memory)} dual objectives. On the other hand, the predicted accuracy in \texttt{(accuracy, latency)} has a moderate correlation ($\tau = 0.5708$), and predicted latency has a strong correlation ($\tau = 0.7542$).

These results indicate a direct relationship between the neural architectures' representations and their desired metrics. Comparatively, hardware cost can be more easily inferred from these architectures than accuracy. This is because the types of operations used in a neural architecture more easily reflect its hardware cost. For example, more convolutional filters in a network will need more computation than fewer convolutional filters \cite{Mih2024}. Such a relationship cannot be directly inferred for accuracy performance, thus explaining the moderate correlation.  


We also observe that for both TSS and SSS search spaces, the correlation of the accuracies is consistent across objective pairs for the same test set, even though the evaluator is trained separately for each pair. For example, in the TSS \texttt{(accuracy, memory)} pair, the correlation is $\tau = 0.5266$ and $\tau = 0.5308$ in the \texttt{(accuracy, latency)}. This indicates convergence in evaluator performance on predicting accuracy. 

% [MORE ANALYSIS INVOLVING THE EVALUATOR]

\subsection{HW-NAS-Bench: NAS-Bench-201 Search Space}
The architectures in NAS-Bench-201 are the same as those in the NATS-Bench topology search space, so we omit training the evaluator on the\texttt{(accuracy, memory)} pair. This is because our estimation of max memory usage will always be constant given the same architecture and input tensor, irrespective of the device.
We rather focus on the latency correlation across the various hardware devices, as latency is more sensitive to the hardware environment. Also, the correlation of true vs. predicted accuracy is provided in Table \ref{}. 

Figure \ref{} shows the plot of true latency vs predicted latency for the NAS-Bench-201 search space for the six edge devices profiled in HW-NAS-Bench. The visualizations show a positive correlation between the predicted and true latency values for all six devices. This implies that the evaluator identifies the relationship between the neural architecture and its latency for each device. However, a cross-device comparison reveals that this relationship is inconsistent, as sampling the same architectures for different devices yields different predictions. 

% The results suggest that hardware design is more crucial for latency than neural architecture design. For the same architectures [assessed], the prediction 

Hardware optimization has a greater impact on edge devices than the neural architecture itself. A heavily optimized device, such as the Edge TPU, is the most optimized for inference latency; thus, the network's latency would be less dependent on its architecture than on hardware optimizations. 


\subsection{Evaluator in a NAS}
The contrast in correlation values observed between accuracy (moderate correlation) and hardware costs (strong correlation) highlights the evaluator's strength as a hardware cost predictor. This strength can be leveraged to supplement NAS approaches with accuracy as their single objective by flexibly adding a hardware constraint to their search strategy. To validate this, we include the SEval-NAS in FreeREA \cite{Cavagnero2023} to search in the NATS-Bench search space and define hardware constraints for the search.  FreeREA uses evolutionary search to find candidate architectures and evaluates the candidate architecture using a training-free metric to estimate the accuracy performance. We include 1) a latency constraint and 2) a memory constraint (searched separately for each constraint) to filter the candidate architectures. For each search, the constraint chosen is the median value of the metric in the dataset.

==> content/temp.tex <==
% \begin{figure}[htbp]
%     \centering
%     % First row with "Memory" label
%     \begin{minipage}{0.05\linewidth}
%         \rotatebox{90}{\fontfamily{phv}\selectfont\large\textbf{\textcolor{violet}{Memory}}} % Vertical label for the first row
%     \end{minipage}
%     \hspace{0pt}% Remove horizontal space between label and subfigures
%     \begin{minipage}{0.9\linewidth}
%         \begin{subfigure}[b]{0.3\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figs/plots/nats_bench/tss_cifar10_memory.png}
%             \caption{CIFAR-10}
%             \label{fig:subfig1}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}[b]{0.3\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figs/plots/nats_bench/tss_cifar100_memory.png}
%             \caption{CIFAR-100}
%             \label{fig:subfig2}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}[b]{0.3\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figs/plots/nats_bench/tss_ImageNet16-120_memory.png}
%             \caption{\scriptsize{ImageNet16-120}}
%             \label{fig:subfig3}
%         \end{subfigure}
%     \end{minipage}

%     % Second row with "Latency" label
%     \begin{minipage}{0.05\linewidth}
%         \rotatebox{90}{\fontfamily{phv}\selectfont\large\textbf{\textcolor{orange}{Latency}}} % Vertical label for the second row
%     \end{minipage}
%     \begin{minipage}{0.9\linewidth}
%         \begin{subfigure}[b]{0.3\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figs/plots/nats_bench/tss_cifar10_latency.png}
%             \caption{CIFAR-10}
%             \label{fig:subfig4}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}[b]{0.3\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figs/plots/nats_bench/tss_cifar100_latency.png}
%             \caption{CIFAR-100}
%             \label{fig:subfig5}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}[b]{0.3\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figs/plots/nats_bench/tss_ImageNet16-120_latency.png}
%             \caption{\scriptsize{ImageNet16-120}}
%             \label{fig:subfig6}
%         \end{subfigure}
%     \end{minipage}

%     \caption{Plots of predicted vs true hardware cost of NATS-Bench TSS architectures (using T5-small) for performance metrics reported on CIFAR-10, CIFAR-100, and ImageNet16-120 datasets. The strength of correlation increases as $\tau$ approaches 1.}
%     \label{fig:plots_nats_tss}
% \end{figure}
% \FloatBarrier

% % \begin{figure}[htbp]
% %     \centering
% %     % \begin{subfigure}[b]{0.3\linewidth}
% %     %     \centering
% %     %     \includegraphics[width=\linewidth]{figs/plots/nats_bench/tss_cifar10_memory.png}
% %     %     \caption{}
% %     %     % \label{fig:subfig1}
% %     % \end{subfigure}
% %     % \hfill
% %     % \begin{subfigure}[b]{0.3\linewidth}
% %     %     \centering
% %     %     \includegraphics[width=\linewidth]{figs/plots/nats_bench/tss_cifar100_memory.png}
% %     %     \caption{}
% %     %     % \label{fig:subfig2}
% %     % \end{subfigure}
% %     % \hfill
% %     % \begin{subfigure}[b]{0.3\linewidth}
% %     %     \centering
% %     %     \includegraphics[width=\linewidth]{figs/plots/nats_bench/tss_ImageNet16-120_memory.png}
% %     %     \caption{}
% %     %     % \label{fig:subfig3}
% %     % \end{subfigure}
    
% %     % \begin{subfigure}[b]{0.3\linewidth}
% %     %     \centering
% %     %     \includegraphics[width=\linewidth]{figs/plots/nats_bench/tss_cifar10_latency.png}
% %     %     \caption{}
% %     %     % \label{fig:subfig4}
% %     % \end{subfigure}
% %     % \hfill
% %     % \begin{subfigure}[b]{0.3\linewidth}
% %     %     \centering
% %     %     \includegraphics[width=\linewidth]{figs/plots/nats_bench/tss_cifar100_latency.png}
% %     %     \caption{}
% %     %     % \label{fig:subfig5}
% %     % \end{subfigure}
% %     % \hfill
% %     % \begin{subfigure}[b]{0.3\linewidth}
% %     %     \centering
% %     %     \includegraphics[width=\linewidth]{figs/plots/nats_bench/tss_ImageNet16-120_latency.png}
% %     %     \caption{}
% %     %     % \label{fig:subfig6}
% %     % \end{subfigure}
% %     \includegraphics[width=\linewidth]{figs/plots/TSS-NATS-Bench.png}
% %     \caption{Plots of predicted vs true hardware cost of NATS-Bench TSS architectures for performance metrics reported on CIFAR-10, CIFAR-100, and ImageNet16-120 datasets. The strength of correlation increases as $\tau$ approaches +1.}
% %     \label{fig:plots_nats_tss}
% % \end{figure}


% \begin{figure}[htbp]
%     \centering
%      % First row with "Memory" label
%     \begin{minipage}{0.05\linewidth}
%         \rotatebox{90}{\fontfamily{phv}\selectfont\large\textbf{\textcolor{violet}{Memory}}} % Vertical label for the first row
%     \end{minipage}\hspace{0pt}% Remove horizontal space between label and subfigures
%     \begin{minipage}{0.92\linewidth}
%         \begin{subfigure}[b]{0.3\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figs/plots/nats_bench/sss_cifar10_memory.png}
%             \caption{CIFAR-10}
%             % \label{fig:subfig1}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}[b]{0.3\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figs/plots/nats_bench/sss_cifar100_memory.png}
%             \caption{CIFAR-100}
%             % \label{fig:subfig2}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}[b]{0.3\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figs/plots/nats_bench/sss_ImageNet16-120_memory.png}
%             % [REDO AFTER TRAINING REDONE]
%             \caption{\scriptsize{ImageNet16-120}}
%             % \label{fig:subfig3}
%         \end{subfigure}
%     \end{minipage}

%     % Second row with "Latency" label
%     \begin{minipage}{0.05\linewidth}
%         \rotatebox{90}{\fontfamily{phv}\selectfont\large\textbf{\textcolor{orange}{Latency}}} % Vertical label for the second row
%     \end{minipage}\hspace{0pt}% Remove horizontal space between label and subfigures
%     \begin{minipage}{0.92\linewidth}  
%         \begin{subfigure}[b]{0.3\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figs/plots/nats_bench/sss_cifar10_latency.png}
%             \caption{CIFAR-10}
%             % \label{fig:subfig4}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}[b]{0.3\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figs/plots/nats_bench/sss_cifar100_latency.png}
%             \caption{CIFAR-100}
%             % \label{fig:subfig5}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}[b]{0.3\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figs/plots/nats_bench/sss_ImageNet16-120_latency.png}
%             % [REDO AFTER TRAINING REDONE]
%             \caption{\scriptsize{ImageNet16-120}}
%             % \label{fig:subfig6}
%         \end{subfigure}
%     \end{minipage}
%     %\includegraphics[width=\linewidth]{figs/plots/SSS-NATS-Bench.png}
%     \caption{Plots of predicted vs true hardware cost of NATS-Bench SSS architectures (using T5-small) for performance metrics reported on CIFAR-10, CIFAR-100, and ImageNet16-120 datasets. The strength of correlation increases as $\tau$ approaches 1.}
%     \label{fig:plots_nats_sss}
% \end{figure}
% \FloatBarrier

% \begin{figure}[htbp]
%     \centering
%     \begin{subfigure}[b]{0.32\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/plots/hw_nas/T5-small_nasbench201_edgegpu.png}
%         \caption{Edge GPU}
%         % \label{fig:subfig1}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.32\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/plots/hw_nas/T5-small_nasbench201_edgetpu.png}
%         \caption{Edge TPU}
%         % \label{fig:subfig2}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.32\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/plots/hw_nas/t5-small_nasbench201_eyeriss.png}
%         % [REDO AFTER TRAINING REDONE]
%         \caption{ASIC Eyeriss}
%         % \label{fig:subfig3}
%     \end{subfigure}
    
%     \begin{subfigure}[b]{0.32\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/plots/hw_nas/t5-small_nasbench201_fpga.png}
%         \caption{FPGA}
%         % \label{fig:subfig4}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.32\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/plots/hw_nas/T5-small_nasbench201_pixel3.png}
%         \caption{Pixel 3}
%         % \label{fig:subfig5}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.32\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/plots/hw_nas/T5-small_nasbench201_raspi4_2.png}
%         % [REDO AFTER TRAINING REDONE]
%         \caption{Raspberry Pi 4}
%         % \label{fig:subfig6}
%     \end{subfigure}
%     % \includegraphics[width=\linewidth]{figs/plots/HW-NAS-Bench.png}
%     \caption{Plots of predicted vs true latency for NAS-Bench-201 architectures with T5-small encoder for 6 edge devices reported in the HW-NAS-Bench benchmark. The strength of correlation increases as $\tau$ approaches 1.}
%     \label{fig:plots_hwnas_small}
% \end{figure}
% \FloatBarrier


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

